An Analytical Framework for Device-to-Device Communication in Cellular Networks

This paper presents a framework that enables characterizing analytically the spectral efficiency achievable by D2D (device-to-device) communication integrated with a cellular network. This framework is based on a stochastic geometry formulation with a novel approach to the modeling of interference and with the added possibility of incorporating exclusion regions to protect cellular receivers from excessive interference from active D2D transmitters. To illustrate the potential of the framework, a number of examples are provided. These examples confirm the potential of D2D communication in situations of strong traffic locality as well as the effectiveness of properly sized exclusion regions.

==> commands.tex <==
% ===========================================================================
% File Name: commands.tex
% File Creation Date: 15.6.1995
% Author: Markku Juntti
% Description: Includes useful commands for Latex edition.
% ===========================================================================


% Theorem-like environments
\newtheorem{defin}{Definition}
\newtheorem{theorem}{Theorem}
\newtheorem{prop}{Proposition}
\newtheorem{lemma}{Lemma}
\newtheorem{corollary}{Corollary}
\newtheorem{alg}{Algorithm}

% Equations, arrays, symbols etc.
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\combin}[2]{\ensuremath{ \left( \ba{c} #1 \\ #2 \ea \right) }}
   % number of combinations, i.e., polynomial expansion factor
\newcommand{\diag}{{\mbox{diag}}}
\newcommand{\herm}{^{\mbox{\scriptsize H}}}  % Hermitian transpose
\newcommand{\sherm}{^{\mbox{\tiny H}}}       % Hermitian for subscripts
\newcommand{\tran}{^{\mbox{\scriptsize T}}}  % transpose
%\newcommand{\gtrless}{>}   % transpose for subscripts
\newcommand{\card}{{\mbox{\textbf{card}}}}

%
%\newcommand{\Nt}{N_\mathrm{t}}
%\newcommand{\Nr}{N_\mathrm{r}}

% Sets of numbers
\newcommand{\vbar}{\raisebox{.17ex}{\rule{.04em}{1.35ex}}}
\newcommand{\vbarind}{\raisebox{.01ex}{\rule{.04em}{1.1ex}}}
\newcommand{\R}{\ifmmode {\rm I}\hspace{-.2em}{\rm R} \else ${\rm I}\hspace{-.2em}{\rm R}$ \fi}
\newcommand{\T}{\ifmmode {\rm I}\hspace{-.2em}{\rm T} \else ${\rm I}\hspace{-.2em}{\rm T}$ \fi}
\newcommand{\N}{\ifmmode {\rm I}\hspace{-.2em}{\rm N} \else \mbox{${\rm I}\hspace{-.2em}{\rm N}$} \fi}
%\newcommand{\B}[1]{\ifmmode {\rm I}\hspace{-.2em}{\rm B}^{#1} \else \mbox{${\rm I}\hspace{-.2em}{\rm B}^{#1}$} \fi}
\newcommand{\B}{\ifmmode {\rm I}\hspace{-.2em}{\rm B} \else \mbox{${\rm I}\hspace{-.2em}{\rm B}$} \fi}
\newcommand{\Hil}{\ifmmode {\rm I}\hspace{-.2em}{\rm H} \else \mbox{${\rm I}\hspace{-.2em}{\rm H}$} \fi}
\newcommand{\C}{\ifmmode \hspace{.2em}\vbar\hspace{-.31em}{\rm C} \else \mbox{$\hspace{.2em}\vbar\hspace{-.31em}{\rm C}$} \fi}
\newcommand{\Cind}{\ifmmode \hspace{.2em}\vbarind\hspace{-.25em}{\rm C} \else \mbox{$\hspace{.2em}\vbarind\hspace{-.25em}{\rm C}$} \fi}
\newcommand{\Q}{\ifmmode \hspace{.2em}\vbar\hspace{-.31em}{\rm Q} \else \mbox{$\hspace{.2em}\vbar\hspace{-.31em}{\rm Q}$} \fi}
%\newcommand{\Z}{\ifmmode {\rm\bf Z} \else \mbox{{\rm\bf Z}} \fi}
\newcommand{\Z}{\ifmmode {\rm Z}\hspace{-.28em}{\rm Z} \else ${\rm Z}\hspace{-.28em}{\rm Z}$ \fi}

% Functions
\newcommand{\sgn}{\mbox {sgn}}
\newcommand{\var}{\mbox {var}}
\newcommand{\E}{\mbox {E}}
\newcommand{\cov}{\mbox {cov}}
\renewcommand{\Re}{\mbox {Re}}
\renewcommand{\Im}{\mbox {Im}}
\newcommand{\cum}{\mbox {cum}}

% Bold-face Greek letters
\renewcommand{\vec}[1]{\bf{#1}}     %equation styles %vector/matrix
%\renewcommand{\vec}[1]{\mbox {\boldmath $#1$}}     %equation styles %vector/matrix
\newcommand{\vecsc}[1]{\mbox {\boldmath \scriptsize $#1$}}     %equation styles %vector/matrix
%\newcommand{\vecsc}[1]{\mbox {\bf \scriptsize #1}}
%\newcommand{\itvec}[1]{\mathbf{#1}}     %equation styles %vector/matrix
\newcommand{\itvec}[1]{\mbox {\boldmath $#1$}}
\newcommand{\itvecsc}[1]{\mbox {\boldmath $\scriptstyle #1$}}
\newcommand{\gvec}[1]{\mbox{\boldmath $#1$}}

\newcommand{\balpha}{\mbox {\boldmath $\alpha$}}
\newcommand{\bbeta}{\mbox {\boldmath $\beta$}}
\newcommand{\bgamma}{\mbox {\boldmath $\gamma$}}
\newcommand{\bdelta}{\mbox {\boldmath $\delta$}}
\newcommand{\bepsilon}{\mbox {\boldmath $\epsilon$}}
\newcommand{\bvarepsilon}{\mbox {\boldmath $\varepsilon$}}
\newcommand{\bzeta}{\mbox {\boldmath $\zeta$}}
\newcommand{\boldeta}{\mbox {\boldmath $\eta$}}
\newcommand{\btheta}{\mbox {\boldmath $\theta$}}
\newcommand{\bvartheta}{\mbox {\boldmath $\vartheta$}}
\newcommand{\biota}{\mbox {\boldmath $\iota$}}
\newcommand{\blambda}{\mbox {\boldmath $\lambda$}}
\newcommand{\bmu}{\mbox {\boldmath $\mu$}}
\newcommand{\bnu}{\mbox {\boldmath $\nu$}}
\newcommand{\bxi}{\mbox {\boldmath $\xi$}}
\newcommand{\bpi}{\mbox {\boldmath $\pi$}}
\newcommand{\bvarpi}{\mbox {\boldmath $\varpi$}}
\newcommand{\brho}{\mbox {\boldmath $\rho$}}
\newcommand{\bvarrho}{\mbox {\boldmath $\varrho$}}
\newcommand{\bsigma}{\mbox {\boldmath $\sigma$}}
\newcommand{\bvarsigma}{\mbox {\boldmath $\varsigma$}}
\newcommand{\btau}{\mbox {\boldmath $\tau$}}
\newcommand{\bupsilon}{\mbox {\boldmath $\upsilon$}}
\newcommand{\bphi}{\mbox {\boldmath $\phi$}}
\newcommand{\bvarphi}{\mbox {\boldmath $\varphi$}}
\newcommand{\bchi}{\mbox {\boldmath $\chi$}}
\newcommand{\bpsi}{\mbox {\boldmath $\psi$}}
\newcommand{\bomega}{\mbox {\boldmath $\omega$}}

% Bold italic Roman letters
%\newcommand{\bolda}{\mbox {\boldmath $a$}}
%\newcommand{\bb}{\mbox {\boldmath $b$}}
%\newcommand{\bc}{\mbox {\boldmath $c$}}
%\newcommand{\bd}{\mbox {\boldmath $d$}}
%\newcommand{\bolde}{\mbox {\boldmath $e$}}
%\newcommand{\boldf}{\mbox {\boldmath $f$}}
%\newcommand{\bg}{\mbox {\boldmath $g$}}
%\newcommand{\bh}{\mbox {\boldmath $h$}}
%\newcommand{\bp}{\mbox {\boldmath $p$}}
%\newcommand{\bq}{\mbox {\boldmath $q$}}
%\newcommand{\br}{\mbox {\boldmath $r$}}
%\newcommand{\bs}{\mbox {\boldmath $s$}}
%\newcommand{\bt}{\mbox {\boldmath $t$}}
%\newcommand{\bu}{\mbox {\boldmath $u$}}
%\newcommand{\bv}{\mbox {\boldmath $v$}}
%\newcommand{\bw}{\mbox {\boldmath $w$}}
%\newcommand{\bx}{\mbox {\boldmath $x$}}
%\newcommand{\by}{\mbox {\boldmath $y$}}
%\newcommand{\bz}{\mbox {\boldmath $z$}}


==> delitest.tex <==
% Copyright 2007 TeX Users Group.
% You may freely use, modify and/or distribute this file.
\typesize=10pt

\input lcdplain.mac

% For CM:

% \def\big#1{{\hbox{$\left#1\vbox to8.5\p@{}\right.\n@space$}}}
% \def\Big#1{{\hbox{$\left#1\vbox to11.5\p@{}\right.\n@space$}}}
% \def\bigg#1{{\hbox{$\left#1\vbox to14.5\p@{}\right.\n@space$}}}
% \def\Bigg#1{{\hbox{$\left#1\vbox to17.5\p@{}\right.\n@space$}}}

% Even bigger sizes than plain provides.
\def\biggg#1{{\hbox{$\left#1\vbox to20.5pt{}\right.$}}}
\def\bigggl{\mathopen\biggg}
\def\bigggr{\mathclose\biggg}
\def\Biggg#1{{\hbox{$\left#1\vbox to23.5pt{}\right.$}}}
\def\Bigggl{\mathopen\Biggg}
\def\Bigggr{\mathclose\Biggg}

% for LucidaNewMath:

% \def\big#1{{\hbox{$\left#1\vbox to8.63\p@{}\right.\n@space$}}}
% \def\Big#1{{\hbox{$\left#1\vbox to11.37\p@{}\right.\n@space$}}}
% \def\bigg#1{{\hbox{$\left#1\vbox to14.13\p@{}\right.\n@space$}}}
% \def\Bigg#1{{\hbox{$\left#1\vbox to16.87\p@{}\right.\n@space$}}}

% Even bigger sizes than plain provides.
\def\biggg#1{{\hbox{$\left#1\vbox to19.62pt{}\right.$}}}
\def\bigggl{\mathopen\biggg}
\def\bigggr{\mathclose\biggg}
\def\Biggg#1{{\hbox{$\left#1\vbox to22.37pt{}\right.$}}}
\def\Bigggl{\mathopen\Biggg}
\def\Bigggr{\mathclose\Biggg}

$$
\Bigggl(\bigggl(\Biggl(\biggl(\Bigl(\bigl(({x})\bigr)\Bigr)\biggr)\Biggr)\bigggr)\Bigggr)
% $$
\quad 
% $$
\Bigggl[\bigggl[\Biggl[\biggl[\Bigl[\bigl[[{x}]\bigr]\Bigr]\biggr]\Biggr]\bigggr]\Bigggr]
% $$
% $$
% \Bigggl\lbrack\bigggl\lbrack\Biggl\lbrack\biggl\lbrack\Bigl\lbrack\bigl\lbrack\lbrack{x}\rbrack\bigr\rbrack\Bigr\rbrack\biggr\rbrack\Biggr\rbrack\bigggr\rbrack\Bigggr\rbrack
% $$
\quad  
% $$
\Bigggl\{\bigggl\{\Biggl\{\biggl\{\Bigl\{\bigl\{\{{x}\}\bigr\}\Bigr\}\biggr\}\Biggr\}\bigggr\}\Bigggr\}
$$
% $$
% \Bigggl\lbrace\bigggl\lbrace\Biggl\lbrace\biggl\lbrace\Bigl\lbrace\bigl\lbrace\lbrace{x}\rbrace\bigr\rbrace\Bigr\rbrace\biggr\rbrace\Biggr\rbrace\bigggr\rbrace\Bigggr\rbrace
% $$

$$
\Bigggl\lmoustache\bigggl\lmoustache\Biggl\lmoustache\biggl\lmoustache\Bigl\lmoustache\bigl\lmoustache\lmoustache{x}\rmoustache\bigr\rmoustache\Bigr\rmoustache\biggr\rmoustache\Biggr\rmoustache\bigggr\rmoustache\Bigggr\rmoustache
% $$
\quad  
% $$
\Bigggl\lceil\bigggl\lceil\Biggl\lceil\biggl\lceil\Bigl\lceil\bigl\lceil\lceil{x}\rceil\bigr\rceil\Bigr\rceil\biggr\rceil\Biggr\rceil\bigggr\rceil\Bigggr\rceil
% $$
\quad  
% $$
\Bigggl\lfloor\bigggl\lfloor\Biggl\lfloor\biggl\lfloor\Bigl\lfloor\bigl\lfloor\lfloor{x}\rfloor\bigr\rfloor\Bigr\rfloor\biggr\rfloor\Biggr\rfloor\bigggr\rfloor\Bigggr\rfloor
$$

$$
\Bigggl\langle\bigggl\langle\Biggl\langle\biggl\langle\Bigl\langle\bigl\langle\langle{x}\rangle\bigr\rangle\Bigr\rangle\biggr\rangle\Biggr\rangle\bigggr\rangle\Bigggr\rangle
% $$
\quad  
% $$
\Bigggl\backslash\bigggl\backslash\Biggl\backslash\biggl\backslash\Bigl\backslash\bigl\backslash\backslash{x}/\bigr/\Bigr/\biggr/\Biggr/\bigggr/\Bigggr/
$$

$$
\Bigggl\lgroup\bigggl\lgroup\Biggl\lgroup\biggl\lgroup\Bigl\lgroup\bigl\lgroup\lgroup{x}\rgroup\bigr\rgroup\Bigr\rgroup\biggr\rgroup\Biggr\rgroup\bigggr\rgroup\Bigggr\rgroup
% $$
\quad  
% $$
\Bigggl\uparrow\bigggl\uparrow\Biggl\uparrow\biggl\uparrow\Bigl\uparrow\bigl\uparrow\uparrow{x}\downarrow\bigr\downarrow\Bigr\downarrow\biggr\downarrow\Biggr\downarrow\bigggr\downarrow\Bigggr\downarrow
$$

$$
\Bigggl\Uparrow\bigggl\Uparrow\Biggl\Uparrow\biggl\Uparrow\Bigl\Uparrow\bigl\Uparrow\Uparrow{x}\Downarrow\bigr\Downarrow\Bigr\Downarrow\biggr\Downarrow\Biggr\Downarrow\bigggr\Downarrow\Bigggr\Downarrow
% $$
\quad  
% $$
\Bigggl\updownarrow\bigggl\updownarrow\Biggl\updownarrow\biggl\updownarrow\Bigl\updownarrow\bigl\updownarrow\updownarrow{x}\Updownarrow\bigr\Updownarrow\Bigr\Updownarrow\biggr\Updownarrow\Biggr\Updownarrow\bigggr\Updownarrow\Bigggr\Updownarrow
$$

$$
\Bigggl\arrowvert\bigggl\arrowvert\Biggl\arrowvert\biggl\arrowvert\Bigl\arrowvert\bigl\arrowvert\arrowvert{x}\Arrowvert\bigr\Arrowvert\Bigr\Arrowvert\biggr\Arrowvert\Biggr\Arrowvert\bigggr\Arrowvert\Bigggr\Arrowvert
% $$
\quad
% $$
\Bigggl\Vert\bigggl\Vert\Biggl\Vert\biggl\Vert\Bigl\Vert\bigl\Vert\Vert{x}\vert\bigr\vert\Bigr\vert\biggr\vert\Biggr\vert\bigggr\vert\Bigggr\vert
% $$
\quad
% $$
\Bigggl\bracevert\bigggl\bracevert\Biggl\bracevert\biggl\bracevert\Bigl\bracevert\bigl\bracevert\bracevert{x}\bracevert\bigr\bracevert\Bigr\bracevert\biggr\bracevert\Biggr\bracevert\bigggr\bracevert\Bigggr\bracevert
$$

\end

